Probability Contracts: Accuracy, Coherence, and Decisions Across LLM Interfaces

Equivalent probability requests can lead to different decisions even when both reports are valid. We introduce probability contracts, a benchmark that connects exact finite-world posteriors, validated event alignment, interface coherence, and failure-aware decision evaluation. Across four model-interface configurations on 1,000 worlds, Kev has lower aggregate canonical posterior error than Jev but larger complement and coarsening residuals; accuracy ordering varies by stratum. Jev's Event and Choice interfaces change the binary action on 32.8% of valid pairs at defer cost 0.10. Post-hoc analyses show that disagreement certifies only 11-52% of mean binary pair error and does not consistently outperform confidence for selection. An action-region characterization and a standard scoring-rule identity explain averaging's expected Brier guarantee relative to random interface selection, but not a decision-loss guarantee at each cost. The loss contrast takes both signs on a 99-cost grid for every configuration; small penalties where both policies beat deferral have pointwise intervals containing zero. Secondary checks specified before collection include a separate 400-root cohort, where Event/Choice effects remain configuration-dependent. A joint surface-order and answer-ID intervention shifts posttrained probabilities. Both bounded reasoning arms yield no valid probability reports, leaving their probability accuracy undefined. Probability contracts make these distinctions measurable by evaluating event semantics, posterior error, coverage, and decision cost together.

==> full_metric_tables_v10.tex <==
\begin{table*}[t]
\caption{Response accounting and canonical accuracy. Valid counts all eligible logical requests; TV and Brier use valid canonical roots (990 for Jev; 1,000 local). Intervals are stratified root-bootstrap intervals.}
\label{tab:fullaccuracy}\centering\small
\resizebox{\textwidth}{!}{\begin{tabular}{lrrrrlll}
\toprule
Configuration & Intended & Eligible & Valid & Rej./unavail. & Posterior TV & Expected Brier & Realized Brier\\
\midrule
Kev & 12,000 & 11,913 & 11,913 & 0/0 & 0.2350 [0.2278, 0.2423] & 0.6333 [0.6229, 0.6436] & 0.6359 [0.6160, 0.6571]\\
Base & 12,000 & 11,913 & 11,913 & 0/0 & 0.3740 [0.3655, 0.3824] & 0.7474 [0.7379, 0.7571] & 0.7530 [0.7332, 0.7739]\\
Posttrained & 12,000 & 11,913 & 11,913 & 0/0 & 0.3202 [0.3124, 0.3280] & 0.6938 [0.6831, 0.7048] & 0.6918 [0.6696, 0.7137]\\
Jev-1.13.0 & 12,000 & 11,913 & 11,849 & 62/2 & 0.2677 [0.2599, 0.2754] & 0.6560 [0.6415, 0.6705] & 0.6469 [0.6094, 0.6851]\\
\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}[t]
\caption{Canonical decisions at defer cost 0.10. Action changes compare event and Choice. Jev uses intended-denominator loss, mapping rejected or unavailable requests to defer.}
\label{tab:fulldecision}\centering\small
\resizebox{\textwidth}{!}{\begin{tabular}{llllll}
\toprule
Configuration & Expected loss & Oracle regret & Defer rate & Minus always defer & Event/Choice changes\\
\midrule
Kev & 0.1090 [0.1054, 0.1131] & 0.0193 [0.0158, 0.0232] & 0.9610 [0.9500, 0.9720] & 0.0090 & 0.1490 [0.1290, 0.1710]\\
Base & 0.1000 [0.1000, 0.1000] & 0.0103 [0.0088, 0.0118] & 1.0000 [1.0000, 1.0000] & 0.0000 & 0.0000 [0.0000, 0.0000]\\
Posttrained & 0.1000 [0.1000, 0.1000] & 0.0103 [0.0088, 0.0118] & 1.0000 [1.0000, 1.0000] & 0.0000 & 0.3420 [0.3210, 0.3630]\\
Jev-1.13.0 & 0.1336 [0.1263, 0.1414] & 0.0438 [0.0366, 0.0515] & 0.8160 [0.7920, 0.8380] & 0.0336 & 0.3280 [0.3020, 0.3540]\\
\bottomrule
\end{tabular}}
\end{table*}

